Short Paper: Atomic Execution is Not Enough for Arbitrage Profit Extraction in Shared Sequencers

There has been a growing interest in shared sequencing solutions, in which transactions for multiple rollups are processed together. Their proponents argue that these solutions allow for better composability and can potentially increase sequencer revenue by enhancing MEV extraction. However, little research has been done on these claims, raising the question of understanding the actual impact of shared sequencing on arbitrage profits, the most common MEV strategy in rollups. To address this, we develop a model to assess arbitrage profits under atomic execution across two Constant Product Market Marker liquidity pools and demonstrate that switching to atomic execution does not always improve profits. We also discuss some scenarios where atomicity may lead to losses, offering insights into why atomic execution may not be enough to convince arbitrageurs and rollups to adopt shared sequencing.

==> Sections/2-background.tex <==
\section{Background}
\label{sec:background}

\begin{itemize}
    \item Rollups
    \item MEV and Arbitrage
    \item Interoperability and shared sequencing
\end{itemize}


==> Sections/3-model-v1.tex <==
\section{Modelling arbitrage extraction}
\label{sec:model}

A key question this work hopes to answer is the impact on profit extraction that an arbitrageur would experience when moving from the status quo (i.e., no interoperability between two rollups) to a shared sequencing solution.

To measure this impact, we consider the atomic execution of swaps across two rollups. In short, this property allows an arbitrageur to bundle two swaps (one for each rollup), guaranteeing that if one of the swaps reverts, the other will also revert.

%To measure this impact, the analysis assesses two separate capabilities shared sequencing solutions may introduce. Firstly, we consider the atomic execution of swaps across two rollups. In short, this property allows an arbitrageur to bundle two swaps (one for each rollup), guaranteeing that if one of the swaps reverts, the other will also revert. We discuss how we model the impact on profit of this capability in Subsection \ref{subsec:atomic_model}.

%Secondly, we consider the inclusion of atomic bridging. With this capability, an arbitrageur can include a bridge operation between the two swaps. With this capability, the arbitrageur does not need to maintain liquidity across different rollups to exploit arbitrage opportunities. Instead, they can use a flash loan on the first chain to fund the first swap, bridge the traded tokens to the second chain, execute the second swap with the bridged tokens, and bridge these newly purchased tokens back to the first chain to close the flash loan. 

%Alternatively, if they already have liquidity and wish to avoid using flash loans, they can still take advantage of atomic bridging by maintaining their entire liquidity in a single chain. Whenever an arbitrage opportunity appears, they can make a bridge operation from their "liquidity" chain to the first chain of the arbitrage strategy, execute the swap on the first chain, bridge the swapped tokens to the second chain, execute the swap on the second chain and finally bridge the resulting tokens from the second chain to the "liquidity" chain.

%We describe how we model the economic benefits of atomic bridging in Subsection \ref{subsec:bridging_model}.


 \subsection{Preliminaries}
\label{subsec:model-preliminaries}

Before describing the model to estimate the impact of cross-rollup atomic swaps, we must define some concepts and variables. We begin by assuming that an arbitrageur identifies an opportunity to arbitrage the pools of the $X\text{-}Y$ token pair in two different rollups, $A$ and $B$.

The arbitrage opportunity is identified at the end of the last sequenced block of each rollup, which occurs at times $t_A$ and $t_B$, respectively. The arbitrageur then submits their transactions to the next block of each rollup (i.e., $(t+1)_A$ and $(t+1)_B$). 

At $t_A$, the $X\text{-}Y$ pool in rollup $A$ has a price of $P_A$ and token reserves of $(x_A, y_A)$, while at $t_B$, the same pool in rollup $B$ has a price of $P_B$ and token reserves of $(x_B, y_B)$. Note that we are considering prices denominated in token $Y$. In other words, $P_A = \nicefrac{y_A}{x_A}$ and $P_B = \nicefrac{y_B}{x_B}$. Without loss of generality, let's assume that $P_A > P_B$.

We further assume that the arbitrageur maintains liquidity on both rollups, which is always kept in a stable asset $S$. The arbitrageur can trade between the stable asset $S$ and the target tokens $X$ and $Y$ in both rollups. 

To simplify the analysis, we assume that token $Y$ has the same price in both rollups, represented as $P^Y$, and that token $X$ is such that there is no arbitrage opportunity between trading with the stable token and the $X\text{-}Y$ pool in each rollup. This means token $X$ will have different prices in each rollup, namely, $P^X_A = P_A \cdot P^Y$ and $P^X_B=P_B \cdot P^Y$. 

In addition, the arbitrageur must pay a fee to trade between the stable and target tokens, which we again assume to be the same in both rollups and for both target tokens. This fee is represented as $f^\text{stable}$

The arbitrageur will perform two bundles (one in each rollup) to extract this arbitrage opportunity. The bundles have the following operations:

\begin{itemize}
    \item Swap bundle $S_B$ in rollup $B$:
    \begin{itemize}
        \item Buy $\Delta y_B$ units of token $Y$ at $P^Y$. The arbitrageur pays $\Delta s_B^- = \Delta y_B \cdot (1-f^\text{stable})\cdot P^Y$ units of the stable token.
        \item Swap the $\Delta y_B$ tokens and receive $\Delta x_B$ units of token $X$ in rollup $B$.
        \item Sell $\Delta x_B$ units of token $X$ at $P^X_A$. The arbitrageur receives $\Delta s_B^+ = \Delta x_B \cdot (1-f^\text{stable})\cdot P^X_A$ units of the stable token.
    \end{itemize}
    \item Swap bundle $S_A$ in rollup $A$:
        \begin{itemize}
        \item Buy $\Delta x_A$ units of token $X$ at $P^X_A$. The arbitrageur pays $\Delta s_A^- = \Delta x_A \cdot (1-f^\text{stable})\cdot P^X_B$ units of the stable token.
        \item Swap the $\Delta x_A$ tokens and receive $\Delta y_A$ units of token $Y$.
        \item Sell $\Delta y_A$ units of token $Y$ at $P^Y$. The arbitrageur receives $\Delta s_A^+ = \Delta y_A \cdot (1-f^\text{stable})\cdot P^Y$ units of the stable token.
    \end{itemize}
\end{itemize}

Additionally, let $\mathcal{F}_{S_A}$ and $\mathcal{F}_{S_B}$ be the random variables representing whether the swaps bundles $S_A$ and $S_B$ (respectively) will fail. These variables take the value 1 if the swap fails and 0 if the swap is successful. Here, we assume that the failure probabilities for each rollup are independent.

Finally, we set $\mathcal{G}_A^s$ and $\mathcal{G}_B^s$ as the random variables representing the total transaction fee cost of swap bundles $S_A$ and $S_B$ respectively if the transaction is successful and $\mathcal{G}_A^f$ and $\mathcal{G}_B^f$ as the random variables representing the total transaction fee cost of swap bundles $S_A$ and $S_B$ respectively if the transaction fails.

We further assume that, under the shared sequencer system, the transaction fee cost of the combined bundles is simply the sum of the costs of submitting the two bundles independently on each rollup. In other words, we are ignoring the margin a share sequencing provider may require to run the service.

\subsection{Profit variables}
\label{subsec:model-profit-vars}

Given the arbitrage opportunity defined above, the profit an arbitrageur will extract is simply the pure profit obtained from the swap bundles $S_A$ and $S_B$, minus the transaction costs.

Let's start with defining the pure bundle profit. If a specific bundle is executed, we can determine its pure profit as the difference between the stable tokens used at the bundle's start and those received at the end. In contrast, the pure profit is zero if the bundle is not executed. Thus, we can define the pure profit of a single bundle $S_i$, with $i \in \{A, B\}$, as:

\begin{equation}
    r_{S_i} = (\Delta s_i^+ - \Delta s_i^-) \cdot (1-\mathcal{F}_{S_i})
\end{equation}
%
Note that we still need to define the number of stable tokens paid and received at each pool -- $\Delta s_A^+$, $\Delta s_A^-$, $\Delta s_B^+$, and $\Delta s_B^-$. We provide the derivation in Section~\ref{subsec:model-trade-sizes}. 
Under the atomic execution regime, if one of the bundles reverts, the other bundle will also revert. Therefore, the pure profit of both bundles, in this case, is:

\begin{equation}
    \mathcal{R}_{\text{atomic}} =
        \begin{cases}
          r_{S_A} + r_{S_B} & \text{if} \quad \mathcal{F}_{S_A}=\mathcal{F}_{S_B}=0\\
          0 & \text{otherwise}
        \end{cases}
\end{equation}

On the other hand, under the independent sequencing regime, one bundle can fail while the other does not. In this regime, the pure profit of both bundles is represented as:

\begin{equation}
    \mathcal{R}_{\text{non-atomic}}= r_{S_A} + r_{S_B}
\end{equation}

The costs follow a similar logic. Under the atomic regime, if one bundle fails, the other will also fail, while under the non-atomic regime, bundles can fail independently. Therefore, we set the cost formulas as follows:

\begin{equation}
\mathcal{C}_{\text{atomic}} =
    \begin{cases}
      \mathcal{G}_A^s + \mathcal{G}_B^s & \text{if} \quad \mathcal{F}_{S_A}=\mathcal{F}_{S_B}=0\\
      \mathcal{G}_A^f + \mathcal{G}_B^f & \text{otherwise}
    \end{cases}
\end{equation}

\begin{equation}
\mathcal{C}_{\text{non-atomic}} = \mathcal{G}_A^s \cdot (1-\mathcal{F}_{S_A}) + \mathcal{G}_A^f \cdot \mathcal{F}_{S_A} + \mathcal{G}_B^s \cdot (1-\mathcal{F}_{S_B}) + \mathcal{G}_B^f \cdot \mathcal{F}_{S_B}
\end{equation}

Now, we only need to define the number of stable tokens paid and received at each pool -- $\Delta s_A^+$, $\Delta s_B^-$, $\Delta s_A^+$, and $\Delta s_B^-$.

\subsection{Trade sizes}
\label{subsec:model-trade-sizes}

In the bundle descriptions of the previous subsection, we already represented $\Delta s_A^+$, $\Delta s_B^-$, $\Delta s_A^+$, and $\Delta s_B^-$ in terms of the target trades $\Delta x_A$, $\Delta x_B$, $\Delta y_A$, and $\Delta y_B$. To derive the trade sizes of two target swaps, we assume that both pools are \glspl{CPMM}, charge the same trading fee $f$, and the arbitrageur will execute the optimal trade (i.e., will size its trade to extract the maximal value from the two target pools). We will also assume that, from the time the arbitrage opportunity is identified to the time the arbitrage trade is executed, no uninformed traders will submit further transactions that shift the prices in the pools.

In the bundle $S_B$, the arbitrageur pays $\Delta y_B$ units of token $Y$ to the pool and must pay a fee of $f$. Here, we consider that the \gls{DEX} is processing fees outside of the pool reserves, which means that when a trader wishes to swap a given amount of tokens and pay $\Delta y$, only part of this payment goes to the pool reserve. Concretely, $(1-f) \Delta y$ is added to the poor reserves while $f \Delta y$ is paid to \glspl{LP}. This is the case for Uniswap~V3 pools, for instance.

We can derive how many $X$ tokens the arbitrageur receives in a trade of $\Delta y_B$ by using the property of \gls{CPMM} pools in which the product of the two token reserves must always be a constant:

\begin{equation}
\label{eq:delta-x-b}
    x_B \cdot y_B = \left[x_B - \Delta x_B\right]\left[y_B + (1-f)\Delta y_B\right]  \Longleftrightarrow \Delta x_B = \frac{x_B(1-f)\Delta y_B}{y_B + (1-f)\Delta y_B}
\end{equation}
%
Thus, if the arbitrageur executes this trade, the price in the pool after the trade will be:

\begin{align}
    P_B^\text{end} &= \frac{y_B +(1-f)\Delta y_B}{x_B - \Delta x_B}=\\
    &= \frac{y_B +(1-f)\Delta y_B}{x_B - \frac{x_B(1-f)\Delta y_B}{y_B + (1-f)\Delta y_B}}=\\
    &= \frac{\left[y_B +(1-f)\Delta y_B\right]^2}{x_B \cdot y_B + x_B(1-f)\Delta y_B - x_B(1-f)\Delta y_B}=\\
    &= \frac{\left[ y_B +(1-f)\Delta y_B \right]^2}{x_B \cdot y_B}
\end{align}
%
Using similar logic for the bundle $S_A$, the arbitrageur pays $\Delta x_A$ units of token $X$ and receives the following units of token $Y$:

\begin{equation}
\label{eq:delta-y-a}
    \Delta y_A = \frac{y_A(1-f)\Delta x_A}{x_A + (1-f)\Delta x_A}
\end{equation}

And, at the end of the trade, the price of the pool will be:

\begin{equation}
    P_A^\text{end} = \frac{x_A \cdot y_A}{\left[ x_A + (1-f)\Delta x_A \right]^2}
\end{equation}
%
When the arbitrageur executes the optimal trades, he will pay in rollup $A$ the same units of $X$ tokens he received in rollup $B$, which means that $\Delta x_A = \Delta x_B$. With this equality and equations \ref{eq:delta-x-b} and \ref{eq:delta-y-a}, we can describe the trade sizes $\Delta x_A$, $\Delta x_B$, and $\Delta y_A$ based on the optimal initial size $\Delta y_B$. As for $\Delta y_B$, the optimal trade occurs when the prices in both pools at the end of the trade are equal, i.e., $P_A^\text{end} = P_B^\text{end}$. We can use this to derive $\Delta y_B$:

\begin{align}
    &P_A^\text{end} = P_B^\text{end} \Longleftrightarrow \\
    &\Longleftrightarrow \frac{x_A \cdot y_A}{\left[ x_A + (1-f)\Delta x_A \right]^2} = 
            \frac{\left[ y_B +(1-f)\Delta y_B \right]^2}{x_B \cdot y_B} \\
%        
    &\Longleftrightarrow \frac{\sqrt{x_A \cdot y_A}}{x_A + (1-f)\Delta x_A} = 
        \frac{y_B +(1-f)\Delta y_B}{\sqrt{x_B \cdot y_B}}\\
%        
    &\Longleftrightarrow \frac{\sqrt{x_A \cdot y_A}}{x_A + (1-f)\frac{x_B(1-f)\Delta y_B}{y_B + (1-f)\Delta y_B}} = 
        \frac{y_B +(1-f)\Delta y_B}{\sqrt{x_B \cdot y_B}}\\
%
    &\Longleftrightarrow \frac{\sqrt{x_A \cdot y_A}}{x_A\left[y_B +(1-f)\Delta y_B\right] + (1-f)x_B(1-f)\Delta y_B} = 
        \frac{1}{\sqrt{x_B \cdot y_B}}\\
%
    &\Longleftrightarrow \frac{\sqrt{x_A \cdot y_A}}{x_A \cdot y_B + x_A(1-f)\Delta y_B + x_B(1-f)^2\Delta y_B} = 
        \frac{1}{\sqrt{x_B \cdot y_B}}\\
%
    &\Longleftrightarrow x_A \cdot y_B + x_A(1-f)\Delta y_B + x_B(1-f)^2\Delta y_B = 
        \sqrt{x_A \cdot y_A \cdot x_B \cdot y_B}\\
%
    &\Longleftrightarrow \Delta y_B = 
        \frac{\sqrt{x_A \cdot y_A \cdot x_B \cdot y_B} - x_A \cdot y_B}{(1-f)x_A + (1-f)^2x_B}
\end{align}

%From Robin: In this case, we are assuming that both pools collect their fees outside of the pool reserves (as is the case with Uniswap V3, for instance). This means that the arbitrageur will choose a trade size such that the marginal prices of the pools after the trades (including trading fees) are equal ($P_1 = P_2$).


